Rare but Severe Neural Machine Translation Errors Induced by Minimal Deletion: An Empirical Study on Chinese and English

We examine the inducement of rare but severe errors in English-Chinese and Chinese-English in-domain neural machine translation by minimal deletion of the source text with character-based models. By deleting a single character, we can induce severe translation errors. We categorize these errors and compare the results of deleting single characters and single words. We also examine the effect of training data size on the number and types of pathological cases induced by these minimal perturbations, finding significant variation. We find that deleting a word hurts overall translation score more than deleting a character, but certain errors are more likely to occur when deleting characters, with language direction also influencing the effect.

==> sections/problem.tex <==
\section{Background and Related Work}
\label{sec:related_work}

We first examine prior studies on error inducement and analysis in
\abr{mt}, with particular focus on Chinese \abr{mt}.

Some previous work on statistical \abr{mt} has explicitly examined
particular idiosyncrasies of Zh-En \abr{mt} models, including tense
errors~\citet{liu-etal-2011-learning} and the \textit{de} error
~\citet{chang2009disambiguating}. Tense errors ostensibly occur due to
the general lack of explicit tense in Chinese. The \textit{de} error
refers to an error that appears with the introduction of the character
\chinese{的} (\textit{de}), which serves many grammatical functions
that the examined models fail to disambiguate.

%% Source sentence with Chinese characters, Pinyin (A pronunciation-based
%% typing system for Chinese) and word by word English translation:\\
% \begin{align*}
%         &\text{\chinese{当地}}& &\text{\chinese{一所}}&
%   &\text{\chinese{名声不佳}}& &\text{\chinese{的}}& &\text{\chinese{中
%       学}}&\\ &\text{dang di}& &\text{yi suo}& &\text{ming sheng bu
%     jia}& &\text{de}& &\text{zhong xue}&\\ &\text{local}& &\text{a}&
%   &\text{reputation}& &\text{DE}& &\text{middle school}&\\
% \end{align*}
    
%% Reference: a local middle school with a bad reputation\\ Translation:
%% a bad reputation of the local secondary school\\

%% In this example, in the Chinese sentence, the noun \chinese{名声不佳}
%% (bad reputation) is before the noun \chinese{中}\chinese{学} (middle
%% school), combined with the word \chinese{的} (DE). The word
%% \chinese{的} indicates that `bad reputation' is to describe `middle
%% school'. However, the translation model does not capture this and
%% fails to learn a correct sentence.

%% The reason is that the word \chinese{的} in Chinese has various other
%% functions besides combining two nouns (e.g., combining adjective and
%% noun, verb and noun, etc.) Therefore, the NMT model often fails to
%% realize the correct grammar and sentence structure.

\citet{vilar-etal-2006-error} taxonomize translation errors into
several categories, including \abr{missing words}, \abr{word order},
\abr{unknown words}, \abr{incorrect words}, etc. We use similar
categories for the errors we generate through term deletion. This
taxonomy does not, however, include focus on severe errors such as
\abr{hallucinations}~\cite{lee2019hallucinations}, ``translations''
which bears no relationship to the source
text. \citet{lee2019hallucinations} show that hallucinations in a
statistical \abr{mt} system can be induced by adding a single token.
However, character-based Transformers, which we use, do not have
``words'' as their vocabulary.

% Most related to our work is \citet{belinkov2018synthetic}, which
% examines the effect on NMT systems of many kinds of perturbations on
% western languages, such as random permutations of the text and common
% human errors.
%% Examples of \abr{hallucination} are shown in \ref{fig:5}.

%% \begin{figure}[h]
%%     \centering
%%     \includegraphics[width=5in]{figures/Hallucination.png}
%%     \caption{Examples of Hallucination. \cite{lee2019hallucinations}}
%%     \label{fig:5}
%% \end{figure}

%% As presented in these examples,


\subsection{NMT hallucinations through deletion}

\citet{lee2019hallucinations} examine \abr{hallucination}s on
\abr{smt} models caused by \textit{adding} new tokens. Most
similarly to our work, \citet{belinkov2018synthetic} investigate how
mistyping sentences causes errors on modern \abr{nmt} models with
several western languages. However, they focus on many kinds of such
errors, e.g., mistyped sentences of a non-native speaker, random
permutations of a word's letters, and common typos. In contrast, we
limit ourselves to one specific type of minimal perturbation---missing
single tokens---which they do not examine.

% \section{Problem approach}

% We need to find a systematic way to examine how \abr{hallucination} could be caused by deleting or replacing words.

% \subsection{Find a model}
% The first step is to find or train a modern NMT model. As indicated above, most modern NMT models are derived from the one proposed by \citet{Bahdanau2015NeuralMT} with minor modifications. Therefore, I will look for a model that is an encoder-decoder system with an attention system and do the tests on it.

% \subsection{Generate attacks}
% Next, I am going to generate attacks on the chosen model. Attacks, or adversarial attacks, is a term used to refer to deceptive inputs in adversarial machine learning \cite{10.1145/2046684.2046692}. The `attacks' I will generate are just modifications of original sentences by DELETION or REPLACEMENT. 

% \subsubsection{Deletion}

% One way of doing DELETION is presented by \citet{feng-etal-2018-pathologies}. In this paper, the authors examined the behavior of NLP models by constantly removing the least important word. The importance of each word is calculated using a gradient approximation method.

% In my research, I will also calculate the importance of each word in the sentence. I will do so by calculating the change of the BLEU score when deleting each word. The word that causes the most decrease in BLEU is the most important one in the sentence. Then, by deleting the most important word, I see if the \abr{hallucination} happens.

% \subsubsection{REPLACEMENT}
% An approach of replacement is described by \citet{10.1145/3377812.3382162}. This paper introduced a method called PatInv. It looks for a word in a sentence and replaces it with one of the same type (e.g., noun, verb) but different meaning.

% In my research, I will also look for a data set whose words are tagged with their types like nouns, verbs, adjectives, etc. Then, instead of replacing the word with the same type, I will replace it with different types (e.g., noun to verb, adjective to preposition). I will even try to replace the word with a nonsense token like `abds'. Hopefully, I will find a specific kind of replacement that would most likely cause \abr{hallucination}.

% \subsection{Identify \abr{hallucination}}

% After generating the attacks and running them on the model, I need to identify \abr{hallucination}. Since I am more likely to use a large data set, the manual check will not work. Therefore, I will try to write a program to pick those translations whose BLEU score is nearly 0. A \abr{hallucination} is most likely to happen in such cases.

% \subsection{Improvement}

% If time permits, after identifying the cases where \abr{hallucination} happens, I will improve the current model regarding this issue.



